An Equivariant Filter for Spacecraft Nonlinear Relative Navigation with Range and Bearing Measurements

Relative navigation is a fundamental task in space proximity operations and autonomous rendezvous. The nonlinear relative orbital dynamics are equivariant and admit a semidirect product Lie group symmetry. This property is used to design an Equivariant Filter (EqF). The filter estimates the relative position and velocity between a chaser spacecraft and a target by lifting the filter dynamics to the group, while respecting the underlying geometry of the problem. Simulations demonstrate the filter's performance and effectiveness.

==> table/maneuvers_metrics.tex <==
{
\sisetup{
  detect-all,
  round-mode=places,
  round-precision=2,
  separate-uncertainty=true,
  output-open-uncertainty = [,
  output-close-uncertainty = ],
}
\begin{table}%[htbp]
    \centering
    \caption{Filter performance metrics, for $t\in[0.1,\,0.25]\,T$}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{
        l  % Trajectory
        l  % Position/Velocity
        S[scientific-notation=true, table-format=1.2e1]  % Mean error
        S[scientific-notation=true, table-format=1.2e1]  % Minimum error
        S[table-format=1.2]  % Mean relative error (%)
        S[table-format=1.2, round-precision=3]  % Minimum relative error (%)
        }
        \toprule
        \multicolumn{2}{c}{} &
        \multicolumn{1}{c}{\shortstack{Mean\\manifold\\error}} &
        \multicolumn{1}{c}{\shortstack{Minimum\\manifold\\error}} &
        \multicolumn{1}{c}{\shortstack{Mean\\relative\\error [\%]}} &
        \multicolumn{1}{c}{\shortstack{Minimum\\relative\\error [\%]}} \\
        \midrule
        
        \multirow{2}{*}{\shortstack{Circum-\\navigation}} 
          & Position & \SI{0.165012}{\meter}            & \SI{0.015727}{\meter}             & 0.052453 & 0.004701 \\
          & Velocity & \SI{0.001409}{\meter\per\second} & \SI{0.000107}{\meter\per\second}  & 0.322467 & 0.021896 \\
        \midrule
        \multirow{2}{*}{\shortstack{R-bar\\Approach}}
          & Position & \SI{0.151307}{\meter}            & \SI{0.014783}{\meter}             & 0.036830 & 0.003578 \\
          & Velocity & \SI{0.001216}{\meter\per\second} & \SI{0.000115}{\meter\per\second}  & 1.532027 & 0.144809 \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:performance_metrics}
\end{table}
}
% {
% \sisetup{
%   detect-all,
%   round-mode=places,
%   round-precision=2,
%   separate-uncertainty=true,
%   output-open-uncertainty = [,
%   output-close-uncertainty = ],
% }
% \begin{table}%[htbp]
%     \centering
%     \caption{Filter performance metrics, for $t\in[0.1,\,0.25]\,\mr{T}$}
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{
%         l  % Trajectory
%         l  % Position/Velocity
%         S[scientific-notation=true, table-format=1.2e1]  % Mean error
%         S[scientific-notation=true, table-format=1.2e1]  % Minimum error
%         S[table-format=1.2]  % Mean relative error (%)
%         S[table-format=1.2, round-precision=3]  % Minimum relative error (%)
%         }
%         \toprule
%         \multicolumn{2}{c}{} &
%         \multicolumn{1}{c}{\shortstack{Mean\\manifold\\error}} &
%         \multicolumn{1}{c}{\shortstack{Minimum\\manifold\\error}} &
%         \multicolumn{1}{c}{\shortstack{Mean\\relative\\error [\%]}} &
%         \multicolumn{1}{c}{\shortstack{Minimum\\relative\\error [\%]}} \\
%         \midrule
        
%         \multirow{2}{*}{\shortstack{Circum-\\navigation}} 
%           & Position & \SI{0.151135}{\meter}            & \SI{0.025678}{\meter}             & 0.048673 & 0.006360 \\
%           & Velocity & \SI{0.002806}{\meter\per\second} & \SI{0.000187}{\meter\per\second}  & 0.629282 & 0.040977 \\
%         \midrule
%         \multirow{2}{*}{\shortstack{R-bar\\Approach}}
%           & Position & \SI{0.153445}{\meter}            & \SI{0.009541}{\meter}             & 0.037161 & 0.002534 \\
%           & Velocity & \SI{0.002945}{\meter\per\second} & \SI{0.000316}{\meter\per\second}  & 3.710120 & 0.397868 \\
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:performance_metrics}
% \end{table}
% }
